Which theories have a measurement problem?

It is shown that any theory that has certain properties has a measurement problem, in the sense that it makes predictions that are incompatible with measurement outcomes being absolute (that is, unique and non-relational). These properties are Bell Nonlocality, Information Preservation, and Local Dynamics. The result is extended by deriving Local Dynamics from No Superluminal Influences, Separable Dynamics, and Consistent Embeddings. As well as explaining why the existing Wigner's-friend-inspired no-go theorems hold for quantum theory, these results also shed light on whether a future theory of physics might overcome the measurement problem. In particular, they suggest the possibility of a theory in which absoluteness is maintained, but without rejecting relativity theory (as in Bohm theory) or embracing objective collapses (as in GRW theory).

==> old_contextuality_bit.tex <==

\paragraph{Contextuality.}




The last of our three properties is \textit{contextuality}.
Our notion of contextuality is based on the one found in \cite{vorob1962consistent, abramsky2011sheaf, abramsky2017contextuality} (and recently generalized in \cite{gogioso2022topology}). \cite{abramsky2017contextuality} captures the idea with a nice slogan:
\begin{quote}
    Contextuality arises where we have a family of data which is \textbf{locally consistent}, but \textbf{globally inconsistent}.
\end{quote}

As an example, consider a typical Bell scenario, in which spacelike separated agents Alice and Bob can each choose to measure one of two variables. 
If the experiment is repeated many times, the resulting data can be described by a conditional probability distribution $p(AB|XY)$, where $X$ and $Y$ are bits that respectively represent Alice's and Bob's choices, and $A$ and $B$ are bits representing their outcomes.
This gives rise to four distributions, corresponding to each choice of both measurements.
One can ask whether all of these four distributions can be seen as arising from the same probability distribution over four variables, one for each local outcome and measurement choice. In other words, one can ask whether there exists a distribution $q(A_0A_1B_0B_1)$ such that the following holds.
\begin{equation} \label{eq:proto_contextuality}
    \begin{split}
        p(A = a, B=b|X=0, Y=0) &= \sum_{A_1B_1}q(A_0=a, A_1, B_0=b, B_1) \\
        p(A = a, B=b|X=0, Y=1) &= \sum_{A_1B_0}q(A_0=a, A_1, B_0, B_1=b) \\
        p(A = a, B=b|X=1, Y=0) &= \sum_{A_0B_1}q(A_0, A_1=a, B_0=b, B_1) \\
        p(A = a, B=b|X=1, Y=1) &= \sum_{A_0B_0}q(A_0, A_1=a, B_0, B_1=b) 
    \end{split}
\end{equation}
If such a distribution does not exist, then $p(AB|XY)$ is called contextual. 
By Fine's theorem \cite{fine1982joint, fine1982hidden}, $p(AB|XY)$ not being contextual is equivalent to it admitting a hidden variable explanation in Bell's sense, so of course quantum theory provides some contextual conditional distributions of this form.

Note that in this scenario, $(A, X)$ and $(B, Y)$ are spacelike separated.
This is important if we want contextuality to indicate nonclassicality \cite{barrett2004non}. 
If we allow Alice's and Bob's systems to interact, then even a classical machine made from cogs and springs could reproduce any $p(AB|XY)$, including one that satisfies (\ref{eq:proto_contextuality}).
On the other hand, if we assume they are spacelike separated, then relativity theory gives us a good reason to believe that they do not interact, in which case contextuality is suggestive of nonclassicality.



Thus we will generalize our definition of contextuality in a way that requires spacelike separation. Consider a conditional probability distribution $p(A_1...A_n|X_1...X_n)$. We say that the distribution is contextual just in case there is no probability distribution of the form $q(A_1^1\ldots A_1^{x_1^{\rm max}}A_2^1 \ldots A_2^{x_2^{\rm max}} \ldots A_n^1 \ldots A_n^{x_n^{\rm max}})$, where $x_i^{{\rm max}}$ is cardinality of $X_i$, whose marginals gives rise to $p(A_1...A_n|X_1...X_n)$. That is,
\begin{equation} \label{prob_contextuality} \tag{C1}
\begin{split}
\not\exists q:\forall x_1 \ldots x_n: \ \ \  &p(A_1=a_1\ldots A_n=a_n|X_1=x_1, \ldots X_n=x_n) \\
       &= \sum_{\overline{A_1^{x_1} \ldots A_n^{x_n}}}  q(A_1^1. \ldots  A_1^{x_1}=a_1 \ldots  A_1^{x_1^{\rm max}} \ldots A_n^1 \ldots A_n^{x_n}=a_n \ldots A_n^{x_n^{\rm max}}), \ \ 
\end{split}
\end{equation}
where $\sum_{\overline{A_1^{x_1} \ldots A_n^{x_n}}}$ denotes a sum over all the variables except for $A_1^{x_1} \ldots A_n^{x_n}$
In a perspectival theory, conditional distributions are represented by circuits with only classical inputs and outputs. For a theory to be contextual, we require that it contains some state $\phi$ on $n$ systems and some classically controlled measurement $T$ that together give rise to a contextual probability distributions in the following way.

\begin{equation}\label{eq:contextuality} \tag{C2}
    p(A_1...A_n|X_1...X_n) \ \ = \tikzfig{contextuality}
\end{equation}
We further require that this circuit admits a valid embedding  $\ce$ such that every triplet $(\ce(S_i), \ce(X_i), \ce(A_i))$ is embedded in a region that is spacelike separated from every other. This completes the definition of contextuality for a theory, which is summarized below.

\begin{definition}[Contextuality.]
A perspectival theory is \textbf{contextual} just in case it contains a circuit diagram of the form (\ref{eq:contextuality}) that admits a valid embedding $\ce$ of each triplet of systems $(\ce(S_i), \ce(X_i), \ce(A_i))$ into spacelike separated regions, and that also gives rise to a conditional distribution satisfying (\ref{prob_contextuality}).
\end{definition}

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{ascending}
    \caption{\textit{Ascending and Descending} by M. C. Escher.}
    \label{fig:ascending}
\end{figure}

The idea of contextuality is illustrated rather beautifully by the prints of M. C. Escher, especially \textit{Ascending and Descending}, reproduced in Figure \ref{fig:ascending}.
Taken on its own, each staircase looks perfectly ordinary and consistent.
But they only fit together in very paradoxical way: starting at the bottom of one of the staircases, one can walk up all four staircases and find oneself back at the bottom of the first them!
But, at least if we take a Euclidean geometry for granted, this leads to a logical contradiction: one cannot move only upwards and yet not increase one's height.
Although each staircase is consistent on its own, it is impossible to unify all four staircases into a consistent whole.

These staircases are in direct analogy with the four distributions (\ref{eq:proto_contextuality} in the Bell scenario that cannot be combined into a single probability distribution over a global assignment of the variables. 
More generally, for any contextual theory, an underlying hidden variable model would have to have a quality reminiscent Escher's staircases.
But contextuality alone doesn't imply that the observed part of a world modelled by the theory would have this same character. 
This is because, by assumption, only one context $x_1 \ldots x_n$ can be measured at a time, meaning that in a simple measurement scenario, the global inconsistency never crosses the boundary from the putative hidden variables to the reality we observe.
But, as the next subsection demonstrates, in any perspectival theory that is information-preserving and has local dynamics, as well as being contextual, this boundary can be crossed. Such theories are suggestive of a radically fragmented world, for which even the observed fragments of reality are inconsistent with each other, like Escher's staircases.


==> old_discussion_bit.tex <==

\section{BIL theories and the absoluteness of observed events: a discussion}

The main theorem shows that any BIL theory is incompatible with the absoluteness of observed events; a metaphysical assumption which says roughly that observable reality is objective and univocal. BIL theories therefore push us to be believe in a fragmented reality, a universe divided into pieces, be they worlds, contexts, perspectives, or whatever. It might be that perfectly reasonable and consistent and even classical story can be told about the events in any particular fragment, but when one tries to combine each story into a consistent meta-narrative, one inevitably fails, and ends up contradicting oneself.

Given how important and interesting it is that quantum theory, and more generally BIL theories push us towards such a radical philosophical conclusion, it is worth understanding deeply how they do so. The first part of doing this is seeing understanding the theorem and its mathematical proof. The second part is to take the mathematics and extract its impBILations for how our concepts fit together: in particular, the concepts of information-preservation, locality, contextuality, reality, and objectivity. This is what this section of the paper aims to do.

Let's start by reminding ourselves of what contextuality is. Roughly, a theory is contextual when it satisfies two properties. The first is that it is impossible, according to the theory, to perform any set of measurements simultaneously. For any single measurement, one must therefore choose which observable one wants to measure, and thereby choose not to measure all the observables that are incompatible with it.

Secondly, it must be impossible to consider all the statistics for each choice of observables as the marginal of some probability distribution over a global assignment of all the observables. Less mathematically, this means that one cannot consider the observed probabilities as arising from the probabilities for getting one or another set of hidden variables, with one variable corresponding to each observable that one can measure. 

So far, nothing here presents a paradox for observed events. The probabilities for these are just the probabilities for whatever compatible set of observables one chooses to measure. One only gets a paradox like Bell did when one supposes that the observed events were caused by hidden variables, one for each observable, which can be thought of as existing simultaneously and thus having a joint probability distribution describing their statistics. Or, more abstractly, one gets a paradox when one supposes that all the statistics for measurements which were not performed by "could" have been can be combined into a consistent hole. But when one does not make these assumptions, one is shielded from paradox for the simple reason that the theory is contextual not just in the second but in the first sense described above: one simply cannot simultaneously measure incompatible observables. This constraint prevents the inconsistency of the hidden variables picture infecting the domain of observed reality: only one of the incompatible "fragments" in that picture can cross the boundary into the observed at one time, because whenever one allows one fragment into observed reality, one thereby keeps the others hidden in either.

At least, that's true when we don't consider supermeasurements. When a superobserver can measure a system that includes an observer has done a measurement, and therefore allowed one fragment to enter her perceptions, it raises the possibility that the observer can find and measure the other, incompatible fragments that remain hidden to the first observer. Now, this will not necessarily be possible, and in particular won't be possible if information can be destroyed in the theory. If information can be destroyed, then we can suppose that the fragments not observed by the first observer are obliterated by her measurement, so they can never even in principle join the realm of the observed, in spite of the best efforts of a powerful superobserver.

But if our theory says that information is preserved, even in the process of measurement, then these fragments must still be around somewhere. In principle, they should be accessible to the superobserver. Information-preservation helps a theory generate a paradox by protecting each fragment from destruction, and thus allowing for the possible that each enter the domain of the observed, hence rendering that domain inconsistent in much the same way as the domain of hidden variables would have to be.

But even if the incompatible fragments remain accessible to superobservers, it is not guaranteed that they can be combined in order to create a paradox within observed reality. This is because contextuality proofs rely not only having incompatible fragments, but also crucially on overlapping fragments. The fragments correspond to sets of compatible observables, and fragments overlap when they share a common observable. The inconsistency of the hidden variable picture arises from the assumption that the variable underlying the common observable takes the same value in both fragments. If inconsistency is going to arise in observed reality, then it is necessary that sets overlapping fragments can be observed, and also that one has a reason to believe (at least given an absoluteness assumption) that the observation corresponding to an observable embedded in some overlapping fragments is the same irrespective of the fragments.

This is the role played by the locality assumption. If a theory is dynamically local, then if a measurement X is spacelike separated to a pair of measurments Y and Z, which themselves are timelike, then one should be able to think of either XY or XZ as simultaneously measurements. And, given that observations are unique and objective, the observed outcome at X should be independent of which pair of measurements it is embedded in.  Thus locality enable us to consider overlapping fragments, with the assumption that the part of observed reality which is contained in the overlap is the same in both fragments. This property, together with information-preservation and locality, ensures that we get a paradox. In other words, it assumes that observed reality itself fragments into different, incompatible, and sometimes overlapping pieces.

So, in summary, contextuality, information-preservation, and locality play the following roles in ensuring that observed reality must consist of a number of inconsistent, overlapping fragments:

	1. contextuality ensures that there is inconsistency in any proposed local hidden variable picture underlying our observations; then
	2. information-preservation ensures that when one fragment from such a picture is measured, the other fragments that are inconsistent are not destroyed in the process, and that these other fragments remain accessible to superobservers; and then finally
	3. locality ensures that inconsistent, overlapping fragments can all me combined into observable reality in a single experiment, implying that observable reality must be fragmented.
	

